A finite basis theorem for the description logic ${\cal ALC}$

The main result of this paper is to prove the existence of a finite basis in the description logic ${\cal ALC}$. We show that the set of General Concept Inclusions (GCIs) holding in a finite model has always a finite basis, i.e. these GCIs can be derived from finitely many of the GCIs. This result extends a previous result from Baader and Distel, which showed the existence of a finite basis for GCIs holding in a finite model but for the inexpressive description logics ${\cal EL}$ and ${\cal EL}_{gfp}$. We also provide an algorithm for computing this finite basis, and prove its correctness. As a byproduct, we extend our finite basis theorem to any finitely generated complete covariety (i.e. any class of models closed under morphism domain, coproduct and quotient, and generated from a finite set of finite models).

==> Theories.tex <==
\section{Theories}
\label{theories}

\begin{definition}[Theories]
Let $\Sigma$ be a signature. A {\bf theory} $Th$ over $\Sigma$ or {\bf $\Sigma$-theory} is a set of formulas in $Sen(\Sigma)$.  This theory is said {\bf positive} when each of its formulas  is positive. \\ Given a theory $Th$, ${\cal I}$ is a {\bf $Th$-model} if for every formula $\varphi \in Th$, ${\cal I} \models \varphi$. \\ Let us note $Mod(Th)$ the full subcategory of $Mod(\Sigma)$ where objects are all the $\Sigma$-models that satisfy the axioms in $Th$.~\footnote{Full means that all the morphisms between two $Th$-models in $Mod(\Sigma)$ are preserved in $Mod(Th)$.} 
\end{definition}

A theory in DL is usually called {\bf knowledge base (KB)} and is divided into two components, the {\bf terminological box (TBox)} that contains all formulas of the form $C \sqsubseteq D$ and $C \equiv D$ and the {\bf assertional box (ABox)} that contains all the formulas of the form $x:C$ and $(x,y):r$. 

\begin{proposition}
\label{terminality}
Every model $\mathcal{I}$ where for every $c \in N_C$, $c^\mathcal{I} = \Delta^\mathcal{I}$ and for every $r \in N_R, r^\mathcal{I} = \Delta^\mathcal{I} \times \Delta^\mathcal{I}$ satisfies every positive formula. 
\end{proposition} 

\begin{proof}
It is obvious to show by structural induction over concept expression that for any positive concept expression $C$, we have $C^\mathcal{I} = \Delta^\mathcal{I}$. 
\end{proof}

In the following, we will note such a model $\mathcal{I}$, $\mathcal{T}_X$ where $X = \Delta^\mathcal{I}$. 

\begin{corollary}
\label{corollary:terminal object}
For every theory $Th$, the TBox of which only contains positive formulas, $Mod(Th)$ has a terminal object.  
\end{corollary}

\begin{proof}
This is the model $\mathcal{T}$ (as in Proposition~\ref{initial and terminal models}).
\end{proof}

We will show in Section~\ref{canonical model} the existence of a {\em semi-initial} model in $Mod(Th)$ (i.e. the morphism between this model and the others is not unique) for theories satisfying some conditions on the form of axioms. 

%In the following, we will study supplementary conditions to impose to theories to get an initial object . 

\begin{definition}[Semantical consequence]
Let $Th$ be a $\Sigma$-theory. A formula $\varphi \in Sen(\Sigma)$ is a {\bf semantical consequence} of $Th$, noted $Th \models \varphi$, if for every $Th$-model ${\cal I}$, ${\cal I} \models \varphi$. %\\ We note $Th^\bullet$ the whole set of semantical consequences of $Th$.
\end{definition}

By Proposition~\ref{terminality}, when dealing with positive formulas, consistency means that the category of models is not restricted to models $\mathcal{T}_X$. 

\begin{definition}[Consistency]
A theory $Th$ is {\bf consistent} if it has a model that, when $Th$ is positive, is not $\mathcal{T}_X$ for some sets $X$. 
\end{definition}

\begin{proposition}
\label{finite loweinem-skolem}
Let $Th$ be a consistent theory. For every set $X$, there exists a $Th$-model $\mathcal{Y}$ with $\Delta^\mathcal{Y} = X$ which is different from $\mathcal{T}_{\Delta^\mathcal{Y}}$ if $Th$ is positive. 
\end{proposition}

\begin{proof}
Let $\mathcal{Z}$  be a $Th$-model such that $\mathcal{Z} \neq \mathcal{T}_W$ for some sets $W$ if $Th$ is positive. Two cases can occur depending on the cardinalities of $X$ and $Z =\Delta^\mathcal{Z}$. First, if $|X| < |Z|$, choose an injective mapping $\mu : X \to Z$ such that:

\begin{enumerate}
\item for every $x \in I$, there exists $v \in X$ such that $\mu(v) = x^\mathcal{Z}$ (it is possible to choose such a $v$ since $|X| < |Z|$), and 
\item for every sub-concept $\exists r.C$ occurring in the TBox of $Th$, for every $v \in X$ such that $\mu(v) \in \exists r.C^\mathcal{Z}$, there exists $v' \in X$ such that $(\mu(v),\mu(v')) \in r^\mathcal{Z}$ and $\mu(v') \in C^\mathcal{Z}$.\footnote{When $I$ or $X$ are infinite (and then so is $Z$), by the choice axiom, such a mapping $\mu$ exists.}
\end{enumerate}

%\begin{itemize}
%\item $\forall x \in I, \mu(x^\mathcal{X}) = x^\mathcal{Z}$;
%\item Let $\Gamma = X \setminus \{x^\mathcal{X}|x \in I\}$. Then, $\mu$ is injective on $\Gamma$. 

%\end{itemize}
Then, let us define $\mathcal{Y}$ by:

\begin{itemize}
\item $\Delta^\mathcal{Y} = X$;
\item $\forall x \in I, x^\mathcal{Y} = \mu^{-1}(x^\mathcal{Z})$ ($\mu^{-1}(x^\mathcal{Z})$ exists by the first condition above on the choice of $\mu$);
\item $\forall c \in N_C, c^\mathcal{Y} = \{v \in X \mid \mu(v) \in c^\mathcal{Z}\}$;
\item $\forall r \in N_R, r^\mathcal{Y} = \{(v,v') \in X \times X \mid (\mu(v),\mu(v')) \in r^\mathcal{Z}\}$ 
\end{itemize}
Obviously, $\mu : \mathcal{Y}\to \mathcal{Z}$ is a morphism. The fact that $\mathcal{Y}$ is a $Th$-model derives from the following lemma:

\begin{lemma}
\label{intermediate lemma}
For every concept $C \in \mathcal{EC}(\Sigma)$, we have:
$$\forall v \in X, v \in C^\mathcal{Y} \Longleftrightarrow \mu(v) \in C^\mathcal{Z}$$
for $Y$ and $Z$ as defined above.
\end{lemma}

\begin{proof}
Let us suppose that in $C$ sub-concepts of the form $\forall r. D$ have been replaced by $(\exists r.D^c)^c$. Therefore, the proof is obtained by structural induction on $C$. The basic cases are obvious. For the induction step, several cases have to be considered:

\begin{itemize}
\item For $C = C_1 @ C_2$ with $@ \in \{\sqcap,\sqcup\}$, the conclusion is obvious.
\item For $C = C'^c$, by the induction hypothesis, we have $\forall v \in X, v {\not \in} {C'}^\mathcal{Y} \Longleftrightarrow \mu(v) {\not \in} {C'}^\mathcal{Z}$, and then  $\forall v \in X, v \in {C'^c}^\mathcal{Y} \Longleftrightarrow \mu(v) \in {C'^c}^\mathcal{Z}$.
\item For $C = \exists r. D$, let  $v \in C^\mathcal{Y}$. This means that there exists $v' \in D^\mathcal{Y}$ such that $(v,v') \in r^\mathcal{Y}$. By the induction hypothesis, $\mu(v') \in D^\mathcal{Z}$. Moreover, by definition of $\mathcal{Y}$, $(\mu(v),\mu(v')) \in r^\mathcal{Z}$. \\ Conversely, let $\mu(v) \in C^\mathcal{Z}$.  By definition, there exists $v' \in X$ such that $(\mu(v),\mu(v')) \in r^\mathcal{Z}$ and $\mu(v') \in D^\mathcal{Z}$, and then by definition of $\mathcal{Y}$ and by the induction hypothesis, $v \in C^\mathcal{Y}$. 
\end{itemize}
\end{proof}

Secondly, suppose that $|Z| \leq |X|$. Then, choose a surjective mapping $\mu : X \to Z$. Then, let us define $\mathcal{Y}$ by:

\begin{itemize}
\item $\Delta^\mathcal{Y} = X$;
\item $\forall x \in I, x^\mathcal{Y} \in \mu^{-1}(x^\mathcal{Z})$;
\item $\forall c \in N_C, c^\mathcal{Y} = \{v \in X \mid \mu(v) \in C^\mathcal{Z}\}$;
\item $\forall r \in N_R, r^\mathcal{Y} = \{(v,v') \mid (\mu(v),\mu(v')) \in r^\mathcal{Z}\}$. 
\end{itemize}
Obviously, $\mu : \mathcal{Z} \to \mathcal{Y}$ is a morphism. Here also, the statement of Lemma~\ref{intermediate lemma} holds. The only point that deserves to be checked is when $C = \exists r. D$. The only if part is similar to the proof in Lemma~\ref{intermediate lemma}. To prove the if part, let us suppose that $\mu(v) \in C^\mathcal{Z}$. By definition, there exists $z \in Z$ such that $(\mu(v),z) \in r^\mathcal{Z}$ and $z \in D^\mathcal{Z}$. $\mu$ being surjective, there exists $v' \in X$ such that $\mu(v') = z$, and then $(v,v') \in r^\mathcal{Y}$. By the induction hypothesis, we have that $v' \in D^\mathcal{Y}$, and then we can conclude that $v \in C^\mathcal{Y}$.  
\end{proof}

\begin{corollary}
For every consistent $\Sigma$-theory $Th$, $Mod(Th)$ has finite models.
\end{corollary}

\begin{proof}
By applying Proposition~\ref{finite loweinem-skolem} to any finite set $X$. 
\end{proof}

The problem is that, given a set $X$, we do not know how to build the model $\mathcal{Y}$ such that it satisfies the axioms of $Th$. In the following, we will study the conditions to impose to theories in order to be able to build such a model $\mathcal{Y}$, the carrier $\Delta^\mathcal{Y}$ of which will be defined from the set of individuals $I$. 

%\begin{definition}[Completeness]
%A $\Sigma$-theory $Th$ is {\bf complete} if, and only if two any $Th$-models ${\cal I}$ and ${\cal I}'$ are logically equivalent, i.e. for every $\varphi \in Sen(\Sigma), {\cal I} \models \varphi \Leftrightarrow {\cal I}' \models \varphi$. 
%\end{definition}

%\begin{proposition}
%A $\Sigma$-theory $Th$ is complete if, and only if both conditions are satisfied:

%\begin{itemize}
%\item $Th$ is consistent;
%\item for every formula $\varphi \in Sen(\Sigma)$, either $Th \models \varphi$ or for every $\mathcal{I} \in Mod(Th)$, $\mathcal{I} {\not \models} \varphi$.
%\end{itemize}
%\end{proposition}

An important notion for our purpose, which is usual in mathematical logic, is the one of free model, i.e. models the proof power of which is equivalent to that of theories they satisfy. 
Here, we restrict this notion to a set of formulas and with respect to a class of models. The reason is, as shown in Section~\ref{canonical model}, that subject to constraints, we will be able to build a canonical model which will be free for both a particular set of formulas and a restricted semantics (i.e. for a subcategory of models). 

\begin{definition}[Freeness]
Let $\mathcal{L} \subseteq Sen(\Sigma)$. Let $\mathcal{C}$ be a class of $\Sigma$-models. 
A $\Sigma$-model $\mathcal{I}$ is {\bf free for $\mathcal{L}$ w.r.t. $\mathcal{C}$} if:
$$\forall \varphi \in \mathcal{L}, \mathcal{I} \models \varphi \Longleftrightarrow (\forall \mathcal{Z} \in \mathcal{C}, \mathcal{Z} \models \varphi)$$
\end{definition}

This notion to be free for a model differs from the one in universal algebra defined as solution of universal problem characterized by a set inclusion, and then is based on the existence and uniqueness of homomorphisms between algebras. Actually, our definition of freeness is connected to a consequence of the definition of freeness in universal algebra. Indeed, in universal algebra,  we can show that for any set of equations $Eq$, there always exists a free algebra according to the standard definition for the class of algebras $Alg(Eq)$ that satisfy $Eq$ and the whole set of equations. This free algebra is the term with variable algebra quotiented by the congruence generated from $Eq$. 

